Over-the-Air Ensemble Inference with Model Privacy

We consider distributed inference at the wireless edge, where multiple clients with an ensemble of models, each trained independently on a local dataset, are queried in parallel to make an accurate decision on a new sample. In addition to maximizing inference accuracy, we also want to maximize the privacy of local models. We exploit the superposition property of the air to implement bandwidth-efficient ensemble inference methods. We introduce different over-the-air ensemble methods and show that these schemes perform significantly better than their orthogonal counterparts, while using less resources and providing privacy guarantees. We also provide experimental results verifying the benefits of the proposed over-the-air inference approach, whose source code is shared publicly on Github.

==> algorithm_ensemble_inference.tex <==


\begin{algorithm}[tb!]
\caption{Over-the-Air Private Ensemble Inference}
%\label{algo:system_model}
\label{algor:model}
\begin{algorithmic}
\Require Trained client model $f_i(\cdot)$ for every client $i$, CIS model $s (\cdot)$, new sample $\vec{x}_t$ at timestep $t$
\Ensure Index of the decided class
\Function{OTA\_Private\_Ensemble}{}
    \State Let $\mathcal{P}_t$ contain each client $i$ with probability $p$, independently
    \ForEach{client $i \in \mathcal{P}_t$ in {\it parallel}}
        \State Client $i$ receives $\vec{x}_t$
        \State Calculate $f_i(\vec{x}_t)$ \Comment{Client Model}
        \State $g_i (\vec{x}_t) = f_i(\vec{x}_t) + \mathcal{N}(\vec{0}, \sigma^{2}/|\mathcal{P}_t| \vec{I}_k)$ \Comment{Add noise}
        \State Transmit $A_t g_i (\vec{x}_t)/h_{i,t}$
    \EndFor
    \State $\vec{z}_t = \vec{n}_t +  A_t \sum_{i\in\mathcal{P}_t}g_i(\vec{x}_t)$ \Comment{Air Sum}
    \State CIS receives $\vec{z}_t$
    \State \Return $s(\vec{z}_t)$ \Comment{CIS Model}
\EndFunction
\end{algorithmic}
\end{algorithm}

==> figure_conditions_cifar10.tex <==

    \pgfplotsset{footnotesize,samples=10}    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
    \definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
    \definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
    \definecolor{color5}{rgb}{0.580392156862745,1.0,0.741176470588235}

    \begin{figure}[t]
    \centering
    \ref*{named}
    \begin{tikzpicture}%[scale=0.87]
    \pgfplotsset{%
    width=.45\textwidth
    }
    \begin{axis}[
    legend columns=4,
    legend entries={\scriptsize Majority Voting $(\epsilon=\infty)$,\scriptsize Belief Summation $(\epsilon=\infty)$,\scriptsize Majority Voting $(\epsilon=1)$,\scriptsize Belief Summation $(\epsilon=1)$},
    legend to name=named,
    %legend style={nodes={scale=0.85, transform shape}},
    log basis x={10},
    log basis y={10},
    tick align=inside,
    tick pos=left,
    x grid style={white!69.0196078431373!black},
    xmin=-2, xmax=10,
    xmode=linear,
    xtick style={color=black},
    y grid style={white!69.0196078431373!black},
    ymin=0.75, ymax=1.0,
    ymode=linear,
    ytick style={color=black},xlabel={\footnotesize Channel SNR (dB)},
    ylabel={\footnotesize Macro-F1},
    max space between ticks=1000pt,
    try min ticks=5,
    grid
    ]
        
        \addplot [densely dotted, very thick, color0, mark=x, mark size=3, mark options={solid}]
        table {
-2	0.8997
0	0.8996
2	0.8996
4	0.8996
6	0.8996
8	0.8996
10	0.8996
12	0.8996
14	0.8996
16	0.8996
18	0.8996
20	0.8996
};
        
        \addplot [densely dashed, very thick, color1, mark=o, mark size=1, mark options={solid}]
        table {
-2	0.9016
0	0.9014
2	0.9014
4	0.9014
6	0.9013
8	0.9013
10	0.9014
12	0.9014
14	0.9013
16	0.9013
18	0.9013
20	0.9013
};
        
        \addplot [densely dotted, very thick, color2, mark=x, mark size=3, mark options={solid}]
        table {
-2	0.8003
0	0.8049
2	0.8087
4	0.8107
6	0.8117
8	0.8127
10	0.8127
12	0.8129
14	0.8129
16	0.8131
18	0.8132
20	0.8134
};
        
        \addplot [densely dashed, very thick, color3, mark=o, mark size=1, mark options={solid}]
        table {
-2	0.7875
0	0.7923
2	0.7964
4	0.7983
6	0.7999
8	0.8007
10	0.8013
12	0.8013
14	0.8016
16	0.8017
18	0.8017
20	0.8019
};
        
        \end{axis}
    \end{tikzpicture}
    %
    \begin{tikzpicture}%[scale=0.87]
    \pgfplotsset{%
    width=.45\textwidth
    }
    \begin{axis}[
    log basis x={10},
    log basis y={10},
    tick align=inside,
    tick pos=left,
    x grid style={white!69.0196078431373!black},
    xmin=0.1, xmax=1.0,
    xmode=linear,
    xtick style={color=black},
    y grid style={white!69.0196078431373!black},
    ymin=0.35, ymax=1.0,
    ymode=linear,
    ytick style={color=black},xlabel={\footnotesize Participation Probabilty $p$},
    ylabel={\footnotesize Macro-F1},
    max space between ticks=1000pt,
    try min ticks=5,
    grid
    ]
        
        \addplot [densely dotted,very thick, color0, mark=x, mark size=3, mark options={solid}]
        table {
0.10	0.8761
0.20	0.8864
0.30	0.8902
0.40	0.8921
0.50	0.8955
0.60	0.8975
0.70	0.8981
0.80	0.8992
0.90	0.8996
1.00	0.8996
};
        
        \addplot [densely dashed,very thick, color1, mark=o, mark size=1, mark options={solid}]
        table {
0.10	0.8846
0.20	0.8920
0.30	0.8935
0.40	0.8963
0.50	0.8985
0.60	0.8995
0.70	0.9004
0.80	0.9015
0.90	0.9015
1.00	0.9014
};
        
        \addplot [densely dotted,very thick, color2, mark=x, mark size=3, mark options={solid}]
        table {
0.10	0.3854
0.20	0.4956
0.30	0.5910
0.40	0.6007
0.50	0.6789
0.60	0.7578
0.70	0.7733
0.80	0.7923
0.90	0.8042
1.00	0.8127
};
        
        \addplot [densely dashed,very thick, color3, mark=o, mark size=1, mark options={solid}]
        table {
0.10	0.3762
0.20	0.4833
0.30	0.5784
0.40	0.5869
0.50	0.6664
0.60	0.7445
0.70	0.7611
0.80	0.7793
0.90	0.7918
1.00	0.8013
};
        
        \end{axis}
    \end{tikzpicture}
    \caption{Comparison of ensemble methods with OAC for varying channel SNR (left) and participation probability $p$ (right) on CIFAR-10 dataset.}
    \label{fig:conditions}
    \vspace{-8pt}
    \end{figure}
        

==> table_comparison.tex <==
\begin{table}[t]
    \centering
    \caption{Comparison with the Baselines}
    \resizebox{0.48\textwidth}{!}{\begin{tabular}{clcccc}
    \toprule
    Privacy & Method & CIFAR-10 & CIFAR-100 & FashionMNIST & IMDB\\ \midrule
\multirow{5}{*}{$\epsilon=\infty$} & Best Client Model & $86.37 {\scriptstyle \pm 0.33}$ & $44.73 {\scriptstyle \pm 1.60}$ & $89.55 {\scriptstyle \pm 0.23}$ & $89.31 {\scriptstyle \pm 0.31}$\\
& Orthogonal Majority Voting & $89.97 {\scriptstyle \pm 0.14}$ & $62.51 {\scriptstyle \pm 0.74}$ & $\mathbf{91.92 {\scriptstyle \pm 0.15}}$ & $90.59 {\scriptstyle \pm 0.06}$\\
& Orthogonal Belief Summation & $90.09 {\scriptstyle \pm 0.12}$ & $\mathbf{63.85 {\scriptstyle \pm 0.60}}$ & $91.91 {\scriptstyle \pm 0.11}$ & $\mathbf{90.64 {\scriptstyle \pm 0.05}}$\\
& Majority Voting with OAC & $89.96 {\scriptstyle \pm 0.14}$ & $62.55 {\scriptstyle \pm 0.67}$ & $\mathbf{91.92 {\scriptstyle \pm 0.13}}$ & $90.62 {\scriptstyle \pm 0.10}$\\
& Belief Summation with OAC & $\mathbf{90.14 {\scriptstyle \pm 0.16}}$ & $63.83 {\scriptstyle \pm 0.59}$ & $91.91 {\scriptstyle \pm 0.13}$ & $\mathbf{90.64 {\scriptstyle \pm 0.07}}$\\
\midrule
\multirow{5}{*}{$\epsilon=1$} & Best Client Model & $12.19 {\scriptstyle \pm 0.22}$ & $1.20 {\scriptstyle \pm 0.05}$ & $12.29 {\scriptstyle \pm 0.30}$ & $53.58 {\scriptstyle \pm 0.32}$\\
& Orthogonal Majority Voting & $22.59 {\scriptstyle \pm 0.10}$ & $2.41 {\scriptstyle \pm 0.14}$ & $23.43 {\scriptstyle \pm 0.55}$ & $65.29 {\scriptstyle \pm 0.23}$\\
& Orthogonal Belief Summation & $22.22 {\scriptstyle \pm 0.13}$ & $2.22 {\scriptstyle \pm 0.12}$ & $23.30 {\scriptstyle \pm 0.55}$ & $64.94 {\scriptstyle \pm 0.24}$\\
& Majority Voting with OAC & $\mathbf{81.27 {\scriptstyle \pm 0.10}}$ & $\mathbf{24.24 {\scriptstyle \pm 0.21}}$ & $\mathbf{84.18 {\scriptstyle \pm 0.21}}$ & $\mathbf{89.32 {\scriptstyle \pm 0.07}}$\\
& Belief Summation with OAC & $80.13 {\scriptstyle \pm 0.24}$ & $20.04 {\scriptstyle \pm 0.24}$ & $83.81 {\scriptstyle \pm 0.22}$ & $89.15 {\scriptstyle \pm 0.08}$\\
\bottomrule
    \end{tabular}}
    \label{tab:comparison}
    \vspace{-10pt}
    \end{table}
